Provably Overwhelming Transformer Models with Designed Inputs

We develop an algorithm which, given a trained transformer model $\mathcal{M}$ as input, as well as a string of tokens $s$ of length $n_{fix}$ and an integer $n_{free}$, can generate a mathematical proof that $\mathcal{M}$ is ``overwhelmed'' by $s$, in time and space $\widetilde{O}(n_{fix}^2 + n_{free}^3)$. We say that $\mathcal{M}$ is ``overwhelmed'' by $s$ when the output of the model evaluated on this string plus any additional string $t$, $\mathcal{M}(s + t)$, is completely insensitive to the value of the string $t$ whenever length($t$) $\leq n_{free}$. Along the way, we prove a particularly strong worst-case form of ``over-squashing'', which we use to bound the model's behavior. Our technique uses computer-aided proofs to establish this type of operationally relevant guarantee about transformer models. We empirically test our algorithm on a single layer transformer complete with an attention head, layer-norm, MLP/ReLU layers, and RoPE positional encoding. We believe that this work is a stepping stone towards the difficult task of obtaining useful guarantees for trained transformer models.

==> _ <==
\section{Evaluating on a Single Layer Model}
\label{sec:model_eval}
We demonstrate our technique on single a single layer transformer trained on \lev{TODO specify exact model and dataset}.
Specifically, given our model, we calculate the worst-case deviation and peak-to-peak difference for the model where the domain has an input restriction with free tokens drawn from a single permutation class as in \cref{sec:perm_invar}.

Then, from \cref{thm:metathm}, if the worst-case deviation is less than half of the peak-to-peak difference, we can prove that the output over any permutation class is the same.

Unlike the prior sections, we consider the first token to always be a BOS token, and, for simplicity, we think of the BOS token as part of the free tokens.
Because our proofs are position invariant, our results still hold even if the first token is the BOS token and not part of the repeated set of tokens.

\subsection{Experimental Setup}
\lev{TODO: j use 100\% and idk}
We train a single-layer transformer model with an embedding dimension of 512, using rotary positional embeddings (RoPE) for position-aware attention. The model includes a parallel feed-forward network with a hidden dimension of 2048 and layer normalization. We train on the AG News dataset, using 45\% of the training split with a batch size of 8 and learning rate of 5e-5 using the Adam optimizer.

For our invariance analysis, we examine a few different input restrictions.
Specifically, we consider
\begin{itemize}
	\item \textbf{Random Permutation Class:} We randomly sample alpha-numeric tokens (including spaces and punctuation) to form $\desSet$
	\item \textbf{Random Sentences:} Using the testing set of AG News, we randomly sample (and, need be concatenate) sentences to form $\desSet$
	\item \textbf{Repeating Tokens:} We repeat the set of tokens for \lev{TODO} (which is \lev{TODO N NUMB} tokens) 
\end{itemize}

In each case, we have a \emph{tunable} number of tokens in $\desSet$.

For the permutation class, we consider the following two cases:
\begin{itemize}
	\item \textbf{Random Permutation Class:} We randomly sample alpha-numeric tokens (including spaces and punctuation) to form $\freeToks$.
		We fix such a string to \lev{TODO copy and paste exact string}
	\item \textbf{Yoda Speech:} We fix the free tokens to be the Yoda speech from Star Wars Episode V: The Empire Strikes Back.
		Specifically, we fix the free tokens to be 
		\begin{quote}
		``Strong in this one, the Force is. Hmmmm, yes. Judge me by my size, do you?'
		\end{quote}
			
	

		repeat the set of tokens for \lev{TODO} (which is \lev{TODO N NUMB} tokens)
\end{itemize}

input sequences of length \lev{INPUT SEQUENCE LENGTH}, where the first token is always the BOS token from the BERT tokenizer vocabulary. We analyze several different permutation classes \lev{DESCRIBE PERMUTATION CLASSES}, each containing \lev{N FREE TOKENS} free tokens and \lev{N REPEATED TOKENS} repeated tokens.
For each permutation class under study, we compute the worst-case deviation and peak-to-peak difference as defined in \cref{sec:perm_invar}. We focus particularly on measuring these quantities at \lev{MEASUREMENT POSITION} in the sequence, as this position \lev{EXPLAIN WHY THIS POSITION}.

\subsection{Results}



\lev{AAA}
\begin{figure}
	\includegraphics{figs/plots/devs_smooth_True.png}
\end{figure}

\begin{enumerate}
	\item Sample random string of tokens $N$ times for $\nctx$ (picture as $\nctx$ grows)
	\item Compute how many times we can prove permutation invariance
	\item Plot
\end{enumerate}


TODO:
\begin{itemize}
	\item Mention that we canosider a starting BOS as part of the free tokens/ perm class
	\item Profit
\end{itemize}


==> sections/__Old/find_k_alg.tex <==
\section{Algorithm for verifying single attention head}

\begin{algorithm}[H]
	\caption{$\softmaxCheck:$ Check the softmax}
	\KwData{$k, \nfree, \aExt, \aDic^{min}, \aDic^{max}, \vExt, \vDic^{min}, \vquery$}
	\KwResult{Verification of $\bot$ or $\top$}
	\lev{We need a \emph{upper bound} on $\aDic$ as well}
	Set
	\[
		w = \frac{\sum_{i\in [k]} \exp(\aDic^{min})}{\sum_{i \in [k]} \exp(\aDic^{max}) +
		\sum_{i \in [\nfree]} \exp(\aExt)}.\;
	\]
	%\lev{Hrmm this kind of implies $w > \half$ so if we get $w$ so large it does not really matter if we have the right associated $v$. Maybe instead of thinking about $\tThresh$ we can phrase it as $\calD_{next}$}\;
 \lev{We need to bound \emph{the subtraction} potential from $\vDic$}
	If $w \cdot \vDic^{min} \geq (1 - w) \cdot \vExt$ return $\top$ otherwise return $\bot$ \;
\end{algorithm}

\begin{algorithm}[H]
	\caption{$\findKRep$: find number of times to repeat token $\tau$ at the end of a free ranging sequence of $\nfree$ tokens to ensure a dictator restriction \lev{We can probably have better bounds vis a vis position by writing an expectation} \lev{re-write in terms of infinity norms}}
	\KwData{$\xQuery, \xDic, \nfree, \klen$}
	\KwResult{Result in $\{\top, \bot\}$}
	Fix $\tQuery = \OneHot(\xQuery), \tDic = \OneHot(\xDic)$	\;
	Let $\pQuery = \OneHot(\nfree + k)$\;
	Let $\aExt = \frac{1}{\sqrt{d}} \max_{i \in [\dVocab]} \left[\tQuery EQK^T E^T \OneHot(i)^T + \norm{\pQuery QK^TP^T}_\infty \right]$ \;
	Let $\aDic^{min} = \frac{1}{\sqrt{d}} \left(\tQuery E_q QK^T E^T \cdot \tDic^T - \norm{\pQuery QK^TP^T}_\infty \right)$ \;
	Let $\aDic^{max} = \frac{1}{\sqrt{d}} \left(\tQuery E_q QK^T E^T \cdot \tDic^T + \norm{\pQuery QK^TP^T}_\infty \right)$ \;
	$\tThresh = \OneHot\left(\arg \max_{i \in [\dVocab]} \tDic \cdot EVOU \cdot \OneHot(i)^T - \norm{PVOU \cdot \OneHot(i)^T}_\infty + \tQuery E_q U \cdot \OneHot(i)^T \right)$ \;
	\lev{TODO: monotonicity theorem necessary}\;
	$\vDic^{min} = \tDic \cdot EVOU \cdot \tThresh^T - \norm{PVOU \cdot \tThresh^T}_\infty + \tQuery E_qU \cdot \tThresh^T$\;
	$\vExt = \max_i \max_j \left(\OneHot(i) \cdot EVOU \cdot \OneHot(j)^T + \norm{PVOU \cdot \OneHot(j)^T}_\infty\right)$\;
	\If{$\vDic^{min} \leq 0$}{
		\Return $\bot$\;
	}
	\Return $\softmaxCheck(k, \nfree, \aExt, \aDic^{min}, \aDic^{max}, \vExt, \vDic^{min})$\;
\end{algorithm}

\subsection{Soundness}

Sketch for proof is using the lemmas below.

\begin{lemma}[Infinity Norm for Positional Encoding Bound]
    Fill in lemma
\end{lemma}
\begin{proof}
    Should be easy \lev{TODO}
\end{proof}

\begin{lemma}[Passing $\softmaxCheck$ line $2$ implies fixing (assuming extremal next-token)]
	Assume that the dictator tokens, $\xDic$, are in location $L \subset [\nfree + k]$ where $|L| = k$ and that for some one hot token, $\vec{t}$, $\tDic \cdot EVOU \cdot \vec{t} + \frac{1}{k} \sum_{\ell \in L} \OneHot(\ell) \cdot PVOU \cdot \vec{t} \geq \vDic^{min}$.
	Also, assume that the token $x$ corresponding to $\vec{t}$ is the maximum of such possible sequences.
	Then if $\softmaxCheck$ return $\top$, we have a dictator sequence where the next token is $x$
\end{lemma}
\begin{proof}
	We begin by noting that	$\vExt$ is the maximum possible value of $(\mathbf{x}E + P_{enc}) VOU \OneHot(j)$ for all possible tokens $j$.
	As such, if $(1 - w) \cdot \vExt < z$ for any $z$, then $(1 - w) \cdot \frac{1}{N} \sum_{a \in N} (T_a \cdot E + P_a \cdot P) VOU \cdot {T'_a}^T < z$ for all settings of tokens $T, T' \subseteq {\{\OneHot(1), \dots \OneHot(\dVocab)\}}^N$ and positions $P \subseteq \{\OneHot(0), \dots \OneHot(\nctx)\}^\nctx$.
	So, if for a token $\vec{t}$, we have that $w \cdot \left[\sum_{i \in L} (\tDic E + \OneHot(L_i)) VOU \cdot \vec{t}^T + \tQuery E_q U \cdot \vec{t} \right] > (1 - w) \cdot \vExt$, then a greedy sampling strategy for the next token will select $\vec{t}$ unless there is a token $\vec{t'}$ where 
	\[
		 \sum_{i \in L} (\tDic E + \OneHot(L_i)) VOU \cdot \vec{t}^T + \tQuery E_q U \cdot \vec{t} > \sum_i (\tDic E + \OneHot(L_i)) VOU \cdot \vec{t}^T + \tQuery E_q U \cdot \vec{t}^T.
	\]
	But then, $\vec{t'}$ is selected irrespective of the non-dictator tokens as well.
	We can also see that 
	\[
		\frac{1}{k} \sum_{i \in L} (\tDic E + \OneHot(L_i)) VOU \cdot \vec{t}^T + \tQuery E_q U \cdot \vec{t}^T \geq \vDic.
	\]
	And so, we have a dictator token.

\end{proof}

\begin{lemma}[Monotonicity of extremal token and $\softmaxCheck$]
	If there is another token which is more likely to be outputted, then the $k$ value should pass even if its smaller
\end{lemma}
\begin{proof}
	Application of the above using $L$...
\end{proof}

\begin{lemma}[Non-extremal next token okay]
	Show how if there is a token with more weight (due to say position reasons) then that's okay)
	Use above lemma
\end{lemma}


\begin{lemma}[Passing $\softmaxCheck$ implies fixing]
	Part of this is assuming all the inputs represent proper bounds \emph{for the predicted token} are correct (does not need to be fixed to the predicted token as monotonicity there)
\end{lemma}

\begin{theorem}[Soundness for $k$]
	Just need to prove that the inputs to $\softmaxCheck$ are indeed extremal
\end{theorem}

\section{Verifying Attention with Parallel Linear Layer}
We will use the following model

\begin{align}
	\mathcal{M}(\textbf{t}) =& \sigma^* 
	       \left( (\tQuery E + \pQuery  P) Q K^T  (P^T + E^T \textbf{x}^T) /\sqrt{d} \right) \cdot (\textbf{x}E+P)VOU + (\tQuery E + \pQuery P)U\\
        &+ \pQuery \cdot \relu((\textbf{x}E + P) A_{enc} + b) A_{dec}
\end{align}

Then,
\begin{align}\label{eq:linlayer}
    \pQuery \cdot \relu((\textbf{x}E + P) A_{enc} + b) A_{dec} = 
    \relu((\tQuery E + \pQuery P) A_{enc} + b) A_{dec}
\end{align}

\cref{eq:linlayer} is fixed by $\pQuery$ and $\tQuery$ being one hot vectors.
We can then use the same technique as before

% TODO: Remove P from inifinty norm (its just VOU)

\lev{TODO: Ask people in AI if sequential or parallel are more popular}

\section{Adding in the Layer Norm}
\lev{Write somewhere that $ \tQuery \cdot \relu(\mathcal{L} \cdot A_{enc} + b) \cdot A_{dec} =  \cdot \relu(\tQuery \cdot \mathcal{L} \cdot A_{enc} + b) \cdot A_{dec}$}
\begin{align*}
	\mathcal{M}(\textbf{t}) =& \sigma^* 
	       \left(\tQuery \mathcal{L} \cdot  Q K^T  \mathcal{L}^T /\sqrt{d} \right) \cdot \mathcal{L} VOU + \tQuery\mathcal{L} U\\
        &+ \tQuery \cdot \relu(\mathcal{L} \cdot A_{enc} + b) \cdot A_{dec}
\end{align*}
where
\[
    \mathcal{L} = LN(\mathbf{x} E + P)
\]
\newcommand{\tild}[1]{\widetilde{#1}}

\lev{Specify normalized normalized all one. Specifify, that everything is entrywise!!...
Maybe fix a column and then write out the operation!}
\newcommand{\LNInp}{\tild{\mathbf{x}}}

We define $LN(\tild{\mathbf{x}})$ as 
\[
	LN(\LNInp) = \frac{\LNInp - \OneMat \cdot \LNInp}{\sqrt{\OneMat \cdot (\LNInp\circ\LNInp) - (\OneMat \cdot \LNInp) \circ (\OneMat \cdot \LNInp) + \eps \cdot \OneMat'}} \cdot \gamma + \beta \cdot \OneMat'
\]

Where $\OneMat \in \mathbb{R}^{\nctx \times \nctx}$ and $\OneMat' \in \mathbb{R}^{\nctx \times \dEmb}$ are the matrices with all ones and $\eps$ is a small constant.

\lev{positional encoding in layer norm make things tricky!}
\lev{Think of layernorm as a left multiplication by a fixed vector/ matrix and fixed offset.}

\lev{I think that bounds here need to bounded in a smarter way. Maybe consider your sequence length of repeated tokens, and then this gives us a much tighter average bound and upper bound for the denominator (simply done by maximizing variance?).}

\subsection{Bounding the Layer Norm Scalars}
Given that layernorm acts \emph{coordinate}-wise (column-wise) in the columns of the input, we can provide bounds per coordinate $c \in [\dEmb]$.

\begin{lemma}[Upper bound on expectation]
	\label{lemma:upperExpBound}
	For a token repeated $\klen$ times with $\nfree$ tokens, the expectation in the layer norm is upper bounded by
	\[
		\frac{\klen \left(\tDic \cdot E \cdot \vec{t}_c^T\right)}{\klen + \nfree} +
			\frac{\nfree \left(\norm{E \cdot \vec{t}_c^T}_\infty\right)}{\klen + \nfree} + \norm{P \cdot \vec{t}_c^T}_\infty.
	\]	
\end{lemma}
\begin{proof}
	The proof follows from a simple expansion expectation and noting that the dictator token is repeated $\klen$ times.
\end{proof}

\begin{lemma}[Lower bound on expectation]
	\label{lemma:lowerExpBound}
	\[
		\frac{\klen \left(\tDic \cdot E \cdot \vec{t}_c^T\right)}{\klen + \nfree} -
			\frac{\nfree \left(\norm{E \cdot \vec{t}_c^T}_\infty\right)}{\klen + \nfree} - \norm{P \cdot \vec{t}_c^T}_\infty.
	\]
\end{lemma}

\begin{lemma}[Upper bound on variance]
	\label{lemma:upperVarBound}
	(Pretty easy by combining bounds on expectation)

	For a token repeated $\klen$ times with $\nfree$ tokens, the variance in the layer norm is upper bounded by
	\[
		AHAHA
	\]
\end{lemma}

\lev{Easier to state lemma below when Layer norm is properly defined column wise}
\lev{add in the epsilon part, epsilon. }
\begin{lemma}[Upper bound on denominator]
    For a token repeated $\klen$ times with $\nfree$ tokens, the denominator in the layer norm is upper bounded by, ignoring the $\eps$,
    % https://stats.stackexchange.com/questions/142651/does-the-uniform-distribution-have-the-greatest-variance-among-all-concave-distr#:~:text=The%20uniform%20distribution%20on%20a,two%20points%20of%20the%20graph).
    \[
	    \frac{\left(\norm{E \cdot \vec{t_c}^T}_\infty + \norm{P \cdot \vec{t_c}^T}_\infty \right)}{\sqrt{3}}.
    \]
\end{lemma}
\begin{proof}
	We first (\lev{TODO: cite}) note that for any random variable bounded in $[-a + b, a + b]$, the standard deviation is at most $a/\sqrt{3}$.
	Then, we can note that the difference between the maximum and minimum of the embedding summed with positional encoding is at most $2(\norm{E \cdot \vec{t_c}^T}_\infty + \norm{P \cdot \vec{t_c}^T}_\infty)$.
 \lev{elaborate a bit maybe?}
\end{proof}

\begin{lemma}[Lower bound on denominator]
	The denominator in the layer norm is lower bounded by, ignoring the $\eps$,
	\[
		AHAHAH %\frac{1}{\sqrt{\nctx}} \sqrt{\sum_{p \in [\nctx]} \left(\min(\vec{t_p} \cdot P \cdot \vec{t_c}^T)\right)^2}
	\]
\end{lemma}
\begin{proof}
	For $E_c = E \cdot \vec{t}_c, P_c = P \cdot \vec{t}_c$, we can rewrite the denominator as the squareroot of
	\begin{align*}
		\OneMat \cdot (xE_c + P_c) \circ (xE_c + P_c) - (\OneMat \cdot (xE_c + P_c)) \circ (\OneMat \cdot (xE_c + P_c)) =& \OneMat \cdot (xE_c \circ xE_c) + \OneMat \cdot (P_c \circ P_c) + 2 \cdot \OneMat \cdot (xE_c \circ P_c)	\\
														 &- (\OneMat \cdot (xE_c))^2 - (\OneMat \cdot P_c)^2 - 2 \cdot (\OneMat xE_c \circ \OneMat P_c).
	\end{align*}
	Then, $\OneMat \cdot(xE_c \circ xE_c) - (\OneMat \cdot xE_c)^2 \geq 0$ and $\OneMat \cdot (P_c \circ P_c) - (\OneMat \cdot P_c)^2$ is a fixed value.

	So, we now must find
	\[
		\min_x (\OneMat \cdot (xE \circ P) - \OneMat xE \circ \OneMat P).
	\]
    \lev{Given series of fixed shifts, can we move the fixed shift back to 0? Look at pairwise differences in $E$ and in $P$ ($O(\dVocab^2$). Write out pairwise matrix, build a bound. Easy to show something about average sequence.
    Worth looking at, is $\beta$ positive? Because otherwise repeated entries get subtracted off}
    \lev{Maybe there is a way to remove the bounds}
\end{proof}

\pagebreak



==> sections/__Old/fixed_output.tex <==
\subsection{From Model Collapse to Fixed Outputs}
\label{sec:fixed_output}
Once we have 



==> sections/__Old/lipbound.tex <==
\section{New Lipschitz Bound for Repeated Token Series}
\lev{Better name...}

Before defining the new Lipschitz bound, we first have to define a notion of norm which makes sense in the context of models.
\begin{definition}[$(2, \infty)$ norm]
Let $X \in \R^{\nctx \times \dEmb}$ be a matrix, then we define a custom norm
\[
	\normCust{X} = \max_{i \in \{1, \ldots, \nctx\}} \norm{X_{i}}_2.
\]
In words, the $(2, \infty)$ norm of a matrix is the maximum $2$-norm of any row in the matrix.
\end{definition}
In words

Key to our result is a new-type of input specific Lipschitz bound

\begin{definition}[$\eps$-Lipschitz Bound]
	Let $f: \R^n \to \R^m$ be a function and $\eps > 0$.
	Then, for any specified norm,
	we say that $f$ is $\eps$-Lipschitz if for all $x \in \R^n$ and $y \in \R^n$ such that $|x - y| \leq \eps$, we have
	\[
		|f(x) - f(y)| \leq C |x - y|
	\]
	for some constant $C$.
\end{definition}

% IDEA: have like \sqrt{n_ctx} of the input be !different! from the repeated token


==> sections/__Old/list_of_ideas.tex <==
\section{List of Ideas}

\begin{itemize}
    \item No go result on how memory is stored to show $.... 2 + 5 =$ and $.... 3 + 4 =$ will fail because the previous will always overwhelm. Generalizes to attn heads in parrallel (pay attention to only a few tokens). Maybe in asymptotic for many heads in serial. Something you can prove w/o making the model very contrived.
    \item Formalize model as dynamical system up to some error
    \item Same model, but if you have long context, then will it still select max (or smthng) at the end? Ask to prove model will produce max on any (or up to a bound). Show something with a state machine type model (like RNNs/ Mamba, etc) or Neural Turing Machines or Reinforcement Learning. For example for max, you can always have the model store some information and that gets passed back into the input.
\end{itemize}

==> sections/__Old/notes.tex <==

\section{A Simple, Single Attention Head Model}


\[\mathcal{M}(\textbf{t}) = \ell(\textbf{t}) = \sigma^* 
 \left ( (x_{\tExt{query}} E + P_{\tExt{query}}) Q K^T  (P^T + E^T \textbf{x}^T) /\sqrt{d} \right ) \cdot (\textbf{x}E+P)VOU + (x_{\tExt{query}}E+P_{\tExt{query}})U\]


\section{Results for $P=0$}
Here we will prove statements about the case $P=0$ with the idea being that these could later be generalized to non-zero and non-trivial positional embeddings $P$.  Taking $P = 0$ our model reduces to:

\[\mathcal{M}(\textbf{t}) = \ell(\textbf{t}) = \sigma^* 
 \left ( (x_{\tExt{query}} E + P_{\tExt{query}}) Q K^T   E^T \textbf{x}^T /\sqrt{d} \right ) \cdot \textbf{x}EVOU + (x_{\tExt{query}}E+P_{\tExt{query}})U\]


 In fact we could even remove the $P_{\tExt{query}}$ but we choose to keep them in for the purposes of forward compatibility to later sections of the definition of the $\vec{a}$ vectors which we now introduce.  

 \begin{definition}[$\vec{a}$]
     Let $\vec{a} \equiv (x_{\tExt{query}} E + P_{\tExt{query}}) Q K^T   E^T$
 \end{definition}

 Then we have:

\[\mathcal{M}(\textbf{t}) = \ell(\textbf{t}) = \sigma^* 
 \left ( \vec{a} \textbf{x}^T /\sqrt{d} \right ) \cdot \textbf{x}EVOU + (x_{\tExt{query}}E+P_{\tExt{query}})U\]


\[ = \frac{1}{|Z|}\sum_{j=1}^{n_{ctx}}  e^{a_j}\left( EVOU \right)_j  +(x_{\tExt{query}}E+P_{\tExt{query}})U \]

Now defining 

\begin{definition}[$\vec{r_j}$]
    Let $\vec{r_j} \equiv \left( EVOU \right)_j$ be the rows of $EVOU$.
\end{definition}

\begin{definition}[$w_j$]
     Let $\vec{w} = \sigma(\vec{a} \mathbf{x}^T / \sqrt{d})$ and we have that $\sum_j w_j = 1$.
    
\end{definition}

Rewriting, we have:

\[\mathcal{M}(\textbf{t}) = \ell(\textbf{t}) =  \sum_{j=1}^{d_{vocab}}  \Tilde{w}_j \vec{r_j} + (x_{\tExt{query}}E+P_{\tExt{query}})U\]
 
 Where $\Tilde{w}_j$ are the aggregated $w_j$'s collected over repeated input tokens so that there are $d_{vocab}$ different $\Tilde{w}_j$'s as opposed to the $n_{ctx}$ different $w_j$'s.  Nonetheless we still have $\sum_{j=1}^{d_{vocab}}\Tilde{w}_j = 1$
     
\begin{claim}
     Imagine that the input sequence to our model is a prefix of t arbitrary tokens, followed by a fixed sequence of tokens repeated k times.  If the positional embedding of our model is $P=0$, then there exists a linear program which can certify, in time that is polynomial in t, k, and the model dimension d, that the model will persist in repeating the repetitive sequence regardless of which tokens are chosen to fill the t prefix spots.
\end{claim}


\begin{proof}
    Proof Outline:  We want to check that 
\end{proof}

\begin{claim}
    Even though the linear program in Claim 1 does not always return a proof for every value of t and k, it gives a proof of all repeated sequences "asymptotically" in the following sense:  If a fixed sequence is repeated indefinitely by model when $t = 0$ and k is sufficiently large, then, for every $t>0$ there exists a sufficiently large $K_t$ such that the linear program from Claim 1 will return a proof of "robust repetitive loop" for every $k > K_t$.
\end{claim}



\section{Model without fixed $x_{\tExt{query}}$ and with $P \neq 0$}
We propose the following algorithm to find $k$ such that repeating a token 

The model now looks the same, but $x_{\tExt{query}}$ is considered to be a variable rather than a constant as in previous sections. 

\[\mathcal{M}(\textbf{t}) = \ell(\textbf{t}) = \sigma^* 
 \left ( (x_{\tExt{query}} E + P_{\tExt{query}}) Q K^T   E^T \textbf{x}^T /\sqrt{d} \right ) \cdot \textbf{x}EVOU + (x_{\tExt{query}}E+P_{\tExt{query}})U\]

\section{$P \neq 0$}


We now consider the model where $P \neq 0$ and, in particular, as written in \url{https://machinelearningmastery.com/a-gentle-introduction-to-positional-encoding-in-transformer-models-part-1/}

\[P \equiv \]

Suppose you have an input sequence of length 
 and require the position of the 
 object within this sequence. The positional encoding is given by sine and cosine functions of varying frequencies:

 
 
 

Here:

k: Position of an object in the input sequence, 

d : Dimension of the output embedding space

P(k,j) : Position function for mapping a position 
 in the input sequence to index 
 of the positional matrix

n: User-defined scalar, set to 10,000 by the authors of Attention Is All You Need.

i: Used for mapping to column indices 
, with a single value of 
 maps to both sine and cosine functions

In the above expression, you can see that even positions correspond to a sine function and odd positions correspond to cosine functions.

\subsection{How we can deal with this}
We can manually inspect the contribution of $P$ to the attention head and the $PVOU$ as in Ref.~\cite{gross2024compact}. Then, we can add $\Delta w_{\max}$ as in Algorithm 3 of Ref.~\cite{gross2024compact}. Unfortuantly, its not as straighforward for us as we are not computing the max.
Within our linear program, we may be able to consider a linear program which somehow ``maximizes'' the error contributed by $P$. We do have to consider though what ``error'' means

\subsubsection{P in the attention}
This depends on how we do the $P = 0$ proof. There is a pretty simple way to do this (with $P = 0$ and $P = 1$). 

Starting with $P = 0$, say our repeated token is $\tau$. Then, within the attention matrix, we look at the value of $EQKE[\tau, \tau]$. 

If $P \neq 0$, we look at the most negative contribution of $PQKE$ and subtract that from $EQKE[\tau, \tau]$

\section{Parallel Attention Heads}

\section{Serial Attention Heads (with the original positional encodings)}
So there are a couple of ways of doing things. Right now, I'll go with ``parrallel'' residuals (feed forward and attention added together rather than in serial)

%https://www.overleaf.com/read/bcqzfnsshnvv#c2ba62
%
%Jason Gross
%to
%Everyone
%06:11 PM
%JG
%https://arxiv.org/abs/2103.16080
%
%https://arxiv.org/abs/2310.07923
%
%
%
%
%For a particular model M, forall A, B, S, M(ASB) != parity(S)
%
%For a particular M, forall A, B, exists S, M(ASB) != parity(S)
%
%https://arxiv.org/abs/2405.14838
%
%For a particular M, forall A, B, #(S st M(ASB) == parity(S)) is sufficiently small
%
%
%
%According to Jason:
%Layernorm is substracting the mean (), and then dividing by epsilon (1e-10) plus root mean square.  Typically layernorm is applied to the embedded token vectors (apply layernorm to xE, and then continue with the usual architecture).  (It may be standard to use layernorm on the xE inside the softmax, but not the one multiplied by VOU....no, actually Jason corrected and said that it is standard to use it on the VOU part as well).  But, xE is matrix, not a vector, so how do we apply layernorm to xE?
%
%Jason is getting this information from these documents:
%
%https://pytorch.org/docs/stable/generated/torch.nn.LayerNorm.html
%
%
%
%
%https://github.com/TransformerLensOrg/TransformerLens/blob/cb5017ad0f30cde0d3ac0b0f863c27fbec964c28/transformer_lens/components/transformer_block.py#L159-L167
%
%see: self.ln1




==> sections/__Old/prob_proof.tex <==
\section{Probabilistic Proof}
\label{sec:single_layer}
In this section we prove the existance of dictator restrictions for single layer neural networks.
We will define some further notation for the proof and algorithm.



==> sections/concrete_case.tex <==
\newcommand{\ModelFinalC}{{\ModelFinal}'}
\newcommand{\eqclassAlgWD}{\texttt{BoundSoftmax}\WD}
\newcommand{\findAlpha}{\texttt{Find}\_\beta}
\newcommand{\findAlphaMin}{\text{Algorithm to find }\ssMinFA}
\newcommand{\findAlphaMax}{\text{Algorithm to find }\ssMaxFA}
\newcommand{\findAlphaMinR}{\text{Algorithm to find }\ssMinRA}
\newcommand{\findAlphaMaxR}{\text{Algorithm to find }\ssMaxRA}
\newcommand{\obj}{\text{objective}}
\newcommand{\freeToks}{\texttt{FreeToks}}

\newcommand{\minBilin}{\texttt{MinBilinear}}
\newcommand{\maxBilin}{\texttt{MaxBilinear}}
\newcommand{\lowerBounds}{\vec{r}^{\min}}
\newcommand{\upperBounds}{\vec{r}^{\max}}

%\subsubsection{Bounding the Encoding Function}
%\label{sec:concrcase}
%We upper bound the worst-case deviation for $\fenc$ using
%bounds on the ``blowup and shift'' in \cref{lem:boundsBS}:
%\begin{lemma}[Worst-case deviation of $\fenc$]
%	\label{lem:WD_fenc}
%	\begin{align*}
%		\WD&(\vec{e}_\nctx \cdot \fenc; \InpSpace \times \blowupSet \shiftSet)_\infty \leq 
%		\\ \max_{t \in [\dVocab]} &
%		\max_{j \in [\dEmb]}
%		\max_{B \in [\vec{0}, B^{\max} - B^{\min}]} \\
%		&\left|X[t] \cdot \Embed \cdot \diag(B) \cdot \vec{e}_j\right| + S_j^{\max} - S_j^{\min}
%	\end{align*}
%	where the inner maximum term can be computed via a simple linear program.
%\end{lemma}
%
%%Finally, we provide an algorithm which bounds the extremal values of the softmax, $\ssMinFB, \ssMaxFB, \ssMinRB, \ssMaxRB$ in \lev{TODO: appendix or not>}.
%%Our algorithm for computing the extremal values of the softmax requires upper and lower bounding a bilinear form: we provide a simple, though non-optimal, algorithm for this task in \cref{fig:bilinOpt} in \cref{sec:appConcrcase}.
%%			Now, we have the bound for $\fenc$, we simply need to bound the extremal values of softmax, $\softSumMinF, \softSumMaxF, \softSumMinR, \softSumMaxR$, to get a bound on the worst-case deviation.
%%			\lev{TODO: alg reference here? I.e. point to lemma/ algorithm}
%
%
%\iffalse
%\begin{figure}[H]
%	\begin{mdframed}
%		$\findAlphaMinR:$%(\desF{\Model})$
%		\begin{itemize}
%			\item Let $\fenc(\vec{e}) = \vec{e} \cdot \Embed \cdot \diag(B) + S$
%			\item For $j \in [s]$, let 
%				\begin{align*}
%					\vec{\ell}[j] = \frac{1}{\sqrt{\dEmb}} 
%					\minBilin\bigg(Q \PosRot_{j, \nctx} K^T, \Embed[\desSet_j] \cdot \diag(B^{\min}) + S^{\min}, \\
%					\Embed[\desSet_j] \cdot \diag(B^{\max}) + S^{\max} \bigg)
%				\end{align*}
%			\item Return $\sum_j \exp\left(\vec{\ell}_j\right)$
%		\end{itemize}
%		$\findAlphaMaxR:$%(\desF{\Model})$
%		\begin{itemize}
%			\item Let $\fenc(\vec{e}) = \vec{e} \cdot \Embed \cdot \diag(B) + S$
%			\item For $j \in [s]$, let 
%				\begin{align*}
%					\vec{\ell}[j] = \frac{1}{\sqrt{\dEmb}} 
%					\maxBilin\bigg(Q \PosRot_{j, \nctx} K^T, \Embed[\desSet_j] \cdot \diag(B^{\min}) + S^{\min}, \\
%					\Embed[\desSet_j] \cdot \diag(B^{\max}) + S^{\max} \bigg)
%				\end{align*}
%			\item Return $\sum_j \exp\left(\vec{\ell}_j\right)$
%		\end{itemize}
%		$\findAlphaMax:$%(\desF{\Model})$
%		\begin{itemize}
%			\item Let $\fenc(\vec{e}) = \vec{e} \cdot \Embed \cdot \diag(B) + S$
%			\item For $j \in (\ndes, \nctx]$, let 
%				\begin{align*}
%					\vec{\ell}[j] = \frac{1}{\sqrt{\dEmb}} \max_{t \in [\dVocab]} 
%					\maxBilin\bigg(Q \PosRot_{j, \nctx} K^T, \Embed[t] \cdot \diag(B^{\min}) + S^{\min}, \\
%					\Embed[t] \cdot \diag(B^{\max}) + S^{\max} \bigg)
%				\end{align*}
%			\item Return $\sum_j \exp\left(\vec{\ell}_j\right)$
%		\end{itemize}
%
%	\end{mdframed}
%	\caption{The algorithm $\findAlpha$ which computes the pre-softmax logits for a given model $\Model$.
%	}
%	\label{fig:find_ell_alg}
%\end{figure}
%
%\fi
%
%%	\begin{algorithm}[H] \label{alg:overwhelmCheckDetLP}
%%		\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
%%		\Input{$\ssMinRB, \ssMaxRB, \ssMaxFB, \softSumMaxR$}
%%		\Output{\lev{TODO}} 
%%		Calculate \begin{align*}
%%			W^{\attn} &= 2 \cdot (\ssMaxRB - \ssMinRB) \cdot \left(\max_{B \in [B^{\min}, B^{\max}]} |E[\desSet, j] \cdot \diag(B)|  + \max(\norm{S^{\min}}_\infty, \norm{S^{\max}}_\infty \right) \\
%%				  &+ 2 \cdot \ssMaxFB \cdot \max_{B, S} \norm{(E B + S) \cdot V}_{\frobInf}
%%		\end{align*}
%%		as in \cref{lem:att_bound}.
%%		\\
%%		Calculate $W = \Lip(\Unembed) \cdot \left(W^{\attn} + \LipMLP_\infty \cdot W^{\fenc} + W^{\fenc}\right)$ 
%%		as per \cref{lem:mlpbound} and 
%%		\\
%%		Calculate $\peakToPeak(\desF{\Model}, \InpSpace)$ by evaluating $\desF{\Model}$ on $X \gets \InpSpace$ \\
%%		\If{
%%		$W < \peakToPeak(\desF{\Model}, \InpSpace) / 2$ }{\Return ``Squashed''
%%	}
%%	\Else{\Return ``Inconclusive''}
%%	\caption{Meta Algorithm for Calculating bound on $\WD(\desF{\Model}, [X])$}
%%\end{algorithm} 
%



==> sections/det_eps_proof.tex <==



==> sections/robust.tex <==
\section{Worst-Case Robustness}
\label{sec:robustness}
So far, we have shown how to decide overwhelmingness for a specific fixed string $s$ where the \emph{location} of the fixed tokens are constant.
However, we note that if we allow for some flexibility in the locations of the fixed tokens, we can \emph{prove} adversarial robustness for the Hamming metric given a specific input!

\begin{definition}[Hamming Metric]
	For input space $\InpSpace^n$, we define the \emph{Hamming metric} $\mathcal{H}(x,y)$ as the number of positions at which the corresponding symbols are different:
	$$
	\mathcal{H}(x,y) = \sum_{i=1}^n \mathbb{I}(x_i \neq y_i)$$
	where $\mathbb{I}$ is the indicator function.
\end{definition}

We can then define the \emph{Hamming ball} of radius $r$ around a string $s$ as the set of strings $x$ such that $\mathcal{H}(x,s) \leq r$.

Finally, we define adversarial robustness as follows:
\lev{TODO; references and the like?}
\begin{definition}[Adversarial Robustness under Hamming Metric]
	Let $\mathcal{M}$ be a transformer model and $s$ a string of tokens.
	We say that $\mathcal{M}$ is \emph{adversarially robust} to $s \in \InpSpace^n$ under the Hamming metric if there exists a radius $r$ such that for all strings $x$ in the Hamming ball of radius $r$ around $s$ and $x[n] = s[n]$, we have:
	$$\mathcal{M}(x) = \mathcal{M}(s)$$
\end{definition}
Though our restriction that $x[n] = s[n]$ may seem arbitrary, we note that in practice, the last token of a string tends to be some ``end of sentence'' token, and so this restriction applies frequently in practice.

We now turn our attention back to the problem of deciding overwhelmingness.
We note that overwhelmingness is a subset of adversarial robustness where the input string $x$ only differs from $s$ in the last $n_{free}$ tokens.
We can then see that \cref{alg:overwhelmCheckDet} only makes use of token positions in determining $\ell^{\min}$ and $\ell^{\max}$.
So, if we can calculate $\ell^{\min}$ and $\ell^{\max}$ in a position-invariant way, we can prove adversarial robustness for the Hamming metric.
Next, notice that \cref{alg:lminlmax} can be generalized to allow for the $\ell^{\min}$ and $\ell^{\max}$ to be calculated over \emph{all} positions in the string.

\lev{TODO: do we generalize this in a nicer way?}




